Off-Chain Micropayment Pool for High-ThroughputBandwidth Sharing Rewards

This paper presents a layer-2 micropayment pool design which supports high-throughput blockchain off-chain payment, designed specifically for the use case of rewarding users who share redundant bandwidth to assist video stream delivery. We analyze the validity and effectiveness of the proposed micropayment pool. Our analysis results demonstrate that the proposed micropayment pool design is better suited for the bandwidth reward use case compared to existing off-chain payment channel solution.

==> Micropayment Pool - Arxiv/sup_materials.tex <==

In addition to creating direct payment channels between view-relay pairs, off-chain “payment networks” may be employed to route payments through intermediate parties.  For example, the Lightning Network is a network of bidirectional payment channels that allows payment to be routed from one payment channel to the next, without trusting the intermediate peers.  However, routing through a payment channel network involves discovering indirect routes between a viewer and a cacher, yet such indirectly routes may not always exist.  Even when an indirect route does exist between the viewer and the cacher, sending micropayments through extra hops adds latency and complexity

%
% ---- Appendix ----
%

\begin{subappendices}
\renewcommand{\thesection}{\Alph{section}}%
% or try \arabic{section}

\section{Semi-Trust Off-Chain Payment Pool}

In addition to facilitating P2P streaming between a viewer and multiple caching nodes, the ledger system according to the present invention has further utility and functionality on video platforms.  For example, end-user viewers may gift content providers and popular influencers directly, or purchase virtual items and goods which can then be gifted to influencers.  Advertisers and brand sponsors may fund their advertising campaigns to automatically reward influencers whose video streams these ads will be displayed in, and optionally, advertisers can reward viewers for their attention to the stream content and advertisements.  End-users can also purchase premium content, virtual goods and other paid products and services.

Moreover, video platform may encourage its users to share bandwidth by paying users based on the bandwidth shared.  In an illustrative example, Alice (i.e., peer A) shares data to peer Bob, Carol, David, etc., and the video platform may reward Alice blockchain tokens through a micropayment pool, with the processing protocol described below, according to some embodiments of the present invention.  In this illustrative embodiment, a Payment Service verifies signed service receipts and tracker authorization, and sends an updated off-chain transaction to relay/cache nodes for eventual on-chain settlement.  
	
Fig. 9 is a diagram 900 illustrating transactions through a resource-orientated micropayment pool established by a content distributor, showing an edge casher 802 Alice receiving off-chain payments for delivering data content to multiple viewers, including 804 Bob and 806 Carol, according to some embodiments of the present invention.  In this particular example, the following steps are performed. 

Step 1. A Tracker 903 peers viewers 802, 804, and 806 together into a group and gives one or more payment authorization certificates to each participating peer.  For example, an authorization certificate auth(Alice, Bob) may be given to Alice, which ensures that peers or viewers can only exchange payments with the viewer groups that the Tracker establishes.

Step 2. Micropayment pool creation: the video platform may create a micropayment pool with a time-lock and a slashable collateral with the Payment Service, using the following exemplary command 920: [Q1: As the creation of the micropayment pool involves submitting  a funding transaction to the THETA blockchain, does the Payment Service/Payment server make the submission, or does the video platform make the submission?  Q2: do the viewer nodes Bob and Carol pay the video platform? If so when and how?]

CreatePool(resourceId, deposit, collateral, duration).

Again, to create the pool, video platform 901 needs to specify a “Resource ID” resourceId that uniquely represents the digital content she intends to retrieve. It may refer to a video file, or a live stream.  The deposit amount needs to be at least the total value of the resource to be retrieved. For instance, if the resource is a video file which is worth 10 tokens, then the deposit has to be at least 10 tokens.  The collateral is required to discourage double spending. If a double spending attempt is detected by the validators of the blockchain, the collateral will be slashed. [Q: since th micropayment pool is created by the video platform or the Payment service, is the double spending protection against them? Or do they have inherent trust of all peer nodes already?] The duration is a time-lock similar to that of a standard payment channel. Any withdrawal from the payment pool has to be before the time-lock expires.  In the case of a live stream, a deleted deposit may be automatically re-filled to avoid any double spend confusion. 

The Payment Service returns information 922 to the video platform 901, including the Merkle proof of the CreatePool() transaction after it has been committed, as well as createPoolTxHash, the transaction hash of the CreatePool() transaction.  Video platform 901 passes the Merkle proof to Alice in a message 924 so Alice is aware of the creation of the micropayment pool.

Step 3. Alice shares data 930 with peer Bob

Step 4. Off-chain micropayments: Bob signs a ServiceReceipt 940 and send it to Alice off-chain in exchange for parts of the specified resource (e.g. a piece of the video file, a live stream segment, etc.).

Step 5. When Alice receives a micropayment receipt from peers it has served, Alice submits it to the Payment Service along with the authorization certificate, as upload data 950.  The Payment Service needs to verify 1) the ServiceReceipt signed by Bob, and 2) the Tracker authorized sharing between Bob and Alice. 

Step 6. Payment Service sends Alice an updated off-chain transaction 960 which accumulates the total payment Alice has received so far, so Alice can submit it as an on-chain transaction 970 to the blockchain anytime and claim the updated balance of the reward 972. 

off-chain transaction may contain the following data:
targetAddress, transferAmount, createPoolTxHash, targetSettlementSequence, Sign(SKA, targetAddress || transferAmount || createPoolTxHash ||  )

On-chain settlement: Either the video platform or Alice can periodically publish the signed transactions to the blockchain any time before the timelock expires to reward Alice with the tokens. ServicePayment transactions that are published may be called “on-chain settlement” transactions.

Note that the recipient peers need to pay for the gas fee for the on-chain settlement transaction. To pay less transaction fees, they would have the incentive to publish on-chain settlements only when necessary, which is beneficial to the scalability of the network.

Also, no on-chain transaction is needed when Alice share video stream with multiple peers simultaneously. In the video streaming context, this means the viewer can switch to any caching node at any time without making an on-chain transaction that could potentially block or delay the video stream delivery.

\section{Applications of Payment Pool Beyond Video Streaming}
	
In the above discussion, the resource-oriented micropayment pool is presented in the video delivery context.  It can be used in other applications as well, as long as a resource can be identified where a user can gain no extra value when he obtains multiple copies of the resource from different peers.  Here are a few examples: a resource can be a generic file, so the resource oriented micropayment pool can facilitate generic file sharing/storage.  In the context of app distribution (e.g. APPLE APPSTORE, GOOGLEPLAY, etc.), an app can be considered as a resource.  A resource can be a certain type of service, e.g., a file compression service, a video transcoding service, solving a set of linear equations, etc. For these services, the requester gains no extra value by getting the same service from two vendors.

\end{subappendices}

==> sup_materials.tex <==

In addition to creating direct payment channels between view-relay pairs, off-chain “payment networks” may be employed to route payments through intermediate parties.  For example, the Lightning Network is a network of bidirectional payment channels that allows payment to be routed from one payment channel to the next, without trusting the intermediate peers.  However, routing through a payment channel network involves discovering indirect routes between a viewer and a cacher, yet such indirectly routes may not always exist.  Even when an indirect route does exist between the viewer and the cacher, sending micropayments through extra hops adds latency and complexity

%
% ---- Appendix ----
%

\begin{subappendices}
\renewcommand{\thesection}{\Alph{section}}%
% or try \arabic{section}

\section{Semi-Trust Off-Chain Payment Pool}

In addition to facilitating P2P streaming between a viewer and multiple caching nodes, the ledger system according to the present invention has further utility and functionality on video platforms.  For example, end-user viewers may gift content providers and popular influencers directly, or purchase virtual items and goods which can then be gifted to influencers.  Advertisers and brand sponsors may fund their advertising campaigns to automatically reward influencers whose video streams these ads will be displayed in, and optionally, advertisers can reward viewers for their attention to the stream content and advertisements.  End-users can also purchase premium content, virtual goods and other paid products and services.

Moreover, video platform may encourage its users to share bandwidth by paying users based on the bandwidth shared.  In an illustrative example, Alice (i.e., peer A) shares data to peer Bob, Carol, David, etc., and the video platform may reward Alice blockchain tokens through a micropayment pool, with the processing protocol described below, according to some embodiments of the present invention.  In this illustrative embodiment, a Payment Service verifies signed service receipts and tracker authorization, and sends an updated off-chain transaction to relay/cache nodes for eventual on-chain settlement.  
	
Fig. 9 is a diagram 900 illustrating transactions through a resource-orientated micropayment pool established by a content distributor, showing an edge casher 802 Alice receiving off-chain payments for delivering data content to multiple viewers, including 804 Bob and 806 Carol, according to some embodiments of the present invention.  In this particular example, the following steps are performed. 

Step 1. A Tracker 903 peers viewers 802, 804, and 806 together into a group and gives one or more payment authorization certificates to each participating peer.  For example, an authorization certificate auth(Alice, Bob) may be given to Alice, which ensures that peers or viewers can only exchange payments with the viewer groups that the Tracker establishes.

Step 2. Micropayment pool creation: the video platform may create a micropayment pool with a time-lock and a slashable collateral with the Payment Service, using the following exemplary command 920: [Q1: As the creation of the micropayment pool involves submitting  a funding transaction to the THETA blockchain, does the Payment Service/Payment server make the submission, or does the video platform make the submission?  Q2: do the viewer nodes Bob and Carol pay the video platform? If so when and how?]

CreatePool(resourceId, deposit, collateral, duration).

Again, to create the pool, video platform 901 needs to specify a “Resource ID” resourceId that uniquely represents the digital content she intends to retrieve. It may refer to a video file, or a live stream.  The deposit amount needs to be at least the total value of the resource to be retrieved. For instance, if the resource is a video file which is worth 10 tokens, then the deposit has to be at least 10 tokens.  The collateral is required to discourage double spending. If a double spending attempt is detected by the validators of the blockchain, the collateral will be slashed. [Q: since th micropayment pool is created by the video platform or the Payment service, is the double spending protection against them? Or do they have inherent trust of all peer nodes already?] The duration is a time-lock similar to that of a standard payment channel. Any withdrawal from the payment pool has to be before the time-lock expires.  In the case of a live stream, a deleted deposit may be automatically re-filled to avoid any double spend confusion. 

The Payment Service returns information 922 to the video platform 901, including the Merkle proof of the CreatePool() transaction after it has been committed, as well as createPoolTxHash, the transaction hash of the CreatePool() transaction.  Video platform 901 passes the Merkle proof to Alice in a message 924 so Alice is aware of the creation of the micropayment pool.

Step 3. Alice shares data 930 with peer Bob

Step 4. Off-chain micropayments: Bob signs a ServiceReceipt 940 and send it to Alice off-chain in exchange for parts of the specified resource (e.g. a piece of the video file, a live stream segment, etc.).

Step 5. When Alice receives a micropayment receipt from peers it has served, Alice submits it to the Payment Service along with the authorization certificate, as upload data 950.  The Payment Service needs to verify 1) the ServiceReceipt signed by Bob, and 2) the Tracker authorized sharing between Bob and Alice. 

Step 6. Payment Service sends Alice an updated off-chain transaction 960 which accumulates the total payment Alice has received so far, so Alice can submit it as an on-chain transaction 970 to the blockchain anytime and claim the updated balance of the reward 972. 

off-chain transaction may contain the following data:
targetAddress, transferAmount, createPoolTxHash, targetSettlementSequence, Sign(SKA, targetAddress || transferAmount || createPoolTxHash ||  )

On-chain settlement: Either the video platform or Alice can periodically publish the signed transactions to the blockchain any time before the timelock expires to reward Alice with the tokens. ServicePayment transactions that are published may be called “on-chain settlement” transactions.

Note that the recipient peers need to pay for the gas fee for the on-chain settlement transaction. To pay less transaction fees, they would have the incentive to publish on-chain settlements only when necessary, which is beneficial to the scalability of the network.

Also, no on-chain transaction is needed when Alice share video stream with multiple peers simultaneously. In the video streaming context, this means the viewer can switch to any caching node at any time without making an on-chain transaction that could potentially block or delay the video stream delivery.

\section{Applications of Payment Pool Beyond Video Streaming}
	
In the above discussion, the resource-oriented micropayment pool is presented in the video delivery context.  It can be used in other applications as well, as long as a resource can be identified where a user can gain no extra value when he obtains multiple copies of the resource from different peers.  Here are a few examples: a resource can be a generic file, so the resource oriented micropayment pool can facilitate generic file sharing/storage.  In the context of app distribution (e.g. APPLE APPSTORE, GOOGLEPLAY, etc.), an app can be considered as a resource.  A resource can be a certain type of service, e.g., a file compression service, a video transcoding service, solving a set of linear equations, etc. For these services, the requester gains no extra value by getting the same service from two vendors.

\end{subappendices}
